Characterizing and Modeling Distributed Training with Transient Cloud GPU Servers

Cloud GPU servers have become the de facto way for deep learning practitioners to train complex models on large-scale datasets. However, it is challenging to determine the appropriate cluster configuration---e.g., server type and number---for different training workloads while balancing the trade-offs in training time, cost, and model accuracy. Adding to the complexity is the potential to reduce the monetary cost by using cheaper, but revocable, transient GPU servers. In this work, we analyze distributed training performance under diverse cluster configurations using CM-DARE, a cloud-based measurement and training framework. Our empirical datasets include measurements from three GPU types, six geographic regions, twenty convolutional neural networks, and thousands of Google Cloud servers. We also demonstrate the feasibility of predicting training speed and overhead using regression-based models. Finally, we discuss potential use cases of our performance modeling such as detecting and mitigating performance bottlenecks.

==> figure-latex/figure_k80_parameter_bottleneck.tex <==
\begin{figure}[t]
        \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ps_bot_k80_1.pdf}
            \caption{ResNet-15 and ResNet-32.}
        \label{subfig:ps_bot:resnet} 
        \end{subfigure}
    \hfill
        \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ps_bot_k80_2.pdf}
            \caption{Shake Shake Small and Big.}
        \label{subfig:ps_bot:shake} 
        \end{subfigure}
        \caption{Training with different sizes of cluster of K80 GPU servers. Using 1 parameter server, adding the slower K80 GPU can achieve linear speedup. }
        \label{fig:ps_bot}
    \end{figure}

==> figure-latex/figure_revocation_uptime.tex <==
\begin{figure*}[t]
        \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{k80_hour_after_starting.pdf}
            \caption{K80 GPU.}
        \label{subfig:uptime_k80} 
        \end{subfigure}
    \hfill
        \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{p100_hour_after_starting.pdf}
            \caption{P100 GPU.}
        \label{subfig:uptime_p100} 
        \end{subfigure}
    \hfill
        \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{v100_hour_after_starting.pdf}
            \caption{V100 GPU.}
        \label{subfig:uptime_v100} 
        \end{subfigure}
        \caption{\textbf{Transient server uptime impact on revocations.} We
        analyzed the revocation events for three types of GPU servers that were
        launched throughout twelve non-consecutive days. We found that
        preemptible servers are more likely to be revoked earlier, e.g., more
        than 55\% \texttt{V100} servers were revoked in the first hour compared to
        97\% in the first 12 hours.}
        \label{fig:revocation_uptime}
    \end{figure*}

==> table-latex/table_lifetime_snapshot.tex <==
\begin{table}[H]
\sf
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{rrrr}
\toprule
\textbf{Region}         & \textbf{GPU server type} & \textbf{Start time}    & \textbf{Termination time} \\ \midrule
europe-west1-b & K80             & 2-18 23:40:34 & 02-19 23:46:59   \\
us-central1-c  & K80             & 2-18 23:39:57 & 2-19 23:18:58    \\
us-east1-c     & K80             & 2-18 23:39:42 & 2-19 23:44:18    \\
us-west1-b     & K80             & 2-18 23:40:18 & 2-20 0:02:33     \\
europe-west1-b & K80             & 9-22 15:01:33 & 9-22 15:09:46    \\
us-east1-c     & K80             & 9-22 14:56:15 & 9-22 15:02:00    \\
us-central1-c  & K80             & 2-18 23:40:01 & 2-19 23:46:19    \\
us-west1-b     & K80             & 2-19 12:07:37 & 2-20 12:11:12    \\
europe-west1-b & P100            & 2-19 22:53:56 & 2-20 9:50:30     \\
us-central1-c  & P100            & 2-19 22:53:33 & 2-20 23:34:00    \\
us-east1-c     & P100            & 2-19 22:53:27 & 2-20 5:32:17     \\
us-west1-b     & P100            & 2-20 9:38:40  & 2-20 14:26:14    \\
europe-west1-b & P100            & 9-15 14:30:37 & 9-16 14:43:55    \\
us-central1-c  & P100            & 9-15 14:32:26 & 9-16 14:48:17    \\
us-east1-c     & P100            & 9-15 14:31:17 & 9-15 14:33:35    \\
us-west1-b     & P100            & 9-15 14:29:21 & 9-15 16:16:45    \\
us-central1-c  & V100            & 9-22 15:09:10 & 9-22 15:11:09    \\
us-west1-b     & V100            & 9-22 15:09:01 & 9-22 18:57:41    \\
asia-east1-c   & V100            & 9-15 14:34:49 & 9-15 15:29:51    \\
europe-west4-a & V100            & 9-15 14:35:51 & 9-15 16:25:49    \\
asia-east1-c   & V100            & 9-15 14:34:57 & 9-15 18:18:06    \\
europe-west4-a & V100            & 9-15 14:36:09 & 9-15 15:36:13    \\
us-central1-c  & V100            & 9-15 14:37:56 & 9-15 14:40:47    \\
us-west1-b     & V100            & 9-15 14:39:11 & 9-15 15:39:40    \\ \bottomrule
\end{tabular}
}
\end{table}

==> table-latex/table_model_checkpoint.tex <==

\begin{table}[H]
    \sf
    \centering 
    \resizebox{0.4\textwidth}{!}{
    \begin{tabular}{@{}rrrrr@{}}
    \toprule
    \textbf{Model}             & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Checkpoint \\ (MB)\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Data File \\ (MB)\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Index File\\ (KB)\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Meta File \\ (MB)\end{tabular}}} \\ \midrule
    \rowcolor[HTML]{EFEFEF} 
    \textbf{ResNet-15}         & 6.27                                                                                    & 5.3                                                                                    & 5.42                                                                                   & 0.97                                                                                   \\
    \rowcolor[HTML]{EFEFEF} 
    \textbf{ResNet-32}         & 15.99                                                                                   & 14.19                                                                                  & 11.05                                                                                  & 1.79                                                                                   \\
    \rowcolor[HTML]{EFEFEF} 
    \textbf{Shake Shake Small} & 26.39                                                                                   & 22.36                                                                                  & 22.07                                                                                  & 4.01                                                                                   \\
    \rowcolor[HTML]{EFEFEF} 
    \textbf{Shake Shake Big}   & 204.04
    & 200.01
    & 22.44
    & 4.01
    \vspace{1mm} \\
    \textbf{Shake Shake-a}     & 9.57                                                                                    & 5.64                                                                                   & 21.03                                                                                  & 3.91                                                                                   \\
    \textbf{ResNet-a}          & 9.26                                                                                    & 8.12                                                                                   & 6.71                                                                                   & 1.13                                                                                   \\
    \textbf{ResNet-b}          & 10.57                                                                                   & 9.25                                                                                   & 7.9                                                                                    & 1.31                                                                                   \\
    \textbf{ResNet-c}          & 12.78                                                                                   & 11.09                                                                                  & 10.41                                                                                  & 1.68                                                                                   \\
    \textbf{ResNet-d}          & 19.21                                                                                   & 17.15                                                                                  & 12.91                                                                                  & 2.05                                                                                   \\
    \textbf{ResNet-e}          & 22.45                                                                                   & 20.12                                                                                  & 14.82                                                                                  & 2.32                                                                                   \\
    \textbf{ResNet-f}          & 28.7                                                                                    & 25.9                                                                                   & 17.94                                                                                  & 2.78                                                                                   \\
    \textbf{Shake Shake-b}     & 26.39                                                                                   & 22.36                                                                                  & 22.07                                                                                  & 4.01                                                                                   \\
    \textbf{ResNet-g}          & 38.85                                                                                   & 35.22                                                                                  & 23.61                                                                                  & 3.61                                                                                   \\
    \textbf{ResNet-h}          & 40.41                                                                                   & 36.49                                                                                  & 25.49                                                                                  & 3.89                                                                                   \\
    \textbf{ResNet-i}          & 48.15                                                                                   & 43.68                                                                                  & 29.26                                                                                  & 4.44                                                                                   \\
    \textbf{ResNet-j}          & 54.26                                                                                   & 49.05                                                                                  & 34.36                                                                                  & 5.18                                                                                   \\
    \textbf{Shake Shake-c}     & 54.19                                                                                   & 50.16                                                                                  & 22.13                                                                                  & 4.01                                                                                   \\
    \textbf{Shake Shake-d}     & 93.33                                                                                   & 89.03                                                                                  & 22.39                                                                                  & 4.01                                                                                   \\
    \textbf{Shake Shake-e}     & 117.61                                                                                  & 112.71                                                                                 & 27.29                                                                                  & 4.87                                                                                   \\
    \textbf{Shake Shake-f}     & 143.01                                                                                  & 138.98                                                                                 & 22.42                                                                                  & 4.01                                                                                   \\ \bottomrule
    \end{tabular}
    }
    \end{table}

==> table-latex/table_model_res.tex <==

\begin{table}[H]
    \sf
    \centering
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{@{}rrrr@{}}
        \toprule
        \textbf{Model}                                    & \multicolumn{1}{l}{\textbf{GFLOPs}} & \textbf{(hidden) layer size} & \multicolumn{1}{l}{\textbf{hidden layer depth}} \\ \midrule
        \rowcolor[HTML]{EFEFEF} 
        {\color[HTML]{333333} \textbf{ResNet-15}}         & 0.59                                & (2, 2, 2)                    & N/A                                             \\
        \rowcolor[HTML]{EFEFEF} 
        {\color[HTML]{333333} \textbf{ResNet-32}}         & 1.54                                & (5, 5, 5)                      & N/A                                             \\
        \rowcolor[HTML]{EFEFEF} 
        {\color[HTML]{333333} \textbf{Shake Shake Small}} & 2.41                                & 32                           & 26                                              \\
        \rowcolor[HTML]{EFEFEF} 
        {\color[HTML]{333333} \textbf{Shake Shake Big}}   & 21.29                               & 96                           & 26                                              \vspace{1mm}\\
        \textbf{Shake Shake-a}                            & 0.62                                & 16                           & 26                                              \\
        \textbf{ResNet-a}                                 & 0.8                                 & (2, 3, 3)                      & N/A                                             \\
        \textbf{ResNet-b}                                 & 1.01                                & (2, 5, 3)                      & N/A                                             \\
        \textbf{ResNet-c}                                 & 1.44                                & (3, 8, 3)                      & N/A                                             \\
        \textbf{ResNet-d}                                 & 1.86                                & (6, 6, 6)                      & N/A                                             \\
        \textbf{ResNet-e}                                 & 2.72                                & (7, 7, 7)                      & N/A                                             \\
        \textbf{ResNet-f}                                 & 2.72                                & (8, 9, 9)                      & N/A                                             \\
        \textbf{Shake Shake-b}                            & 3.05                                & 32                           & 32                                              \\
        \textbf{ResNet-g}                                 & 3.67                                & (10, 13, 12)                   & N/A                                             \\
        \textbf{ResNet-h}                                 & 3.99                                & (11, 15, 12)                   & N/A                                             \\
        \textbf{ResNet-i}                                 & 4.63                                & (14, 15, 15)                   & N/A                                             \\
        \textbf{ResNet-j}                                & 5.48                                & (16, 20, 16)                   & N/A                                             \\
        \textbf{Shake Shake-c}                            & 5.37                                & 48                           & 26                                              \\
        \textbf{Shake Shake-d}                            & 9.51                                & 64                           & 26                                              \\
        \textbf{Shake Shake-e}                            & 12.06                               & 64                           & 32                                              \\
        \textbf{Shake Shake-f}                            & 14.81                               & 80                           & 26                                              \\ \bottomrule
        \end{tabular}
    }
    \end{table}

==> table-latex/table_training_speed_snapshot.tex <==
\begin{table}[H]
\sf
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{rrrr}
\toprule
\textbf{GPU Type} & \textbf{GPU TFLOP/S} & \textbf{Model FLOPs} & \textbf{Step Time (s)} \\ \midrule
K80      & 4.113      & 860117021   & 0.130999009   \\
K80      & 4.113      & 1087710757  & 0.154182808   \\
K80      & 4.113      & 1542543029  & 0.200066016   \\
K80      & 4.113      & 2343835089  & 0.290524202   \\
K80      & 4.113      & 2915531621  & 0.347456001   \\
K80      & 4.113      & 10208089582 & 0.784177734   \\
P100     & 9.526      & 860117021   & 0.058104989   \\
P100     & 9.526      & 1087710757  & 0.068521969   \\
P100     & 9.526      & 1542543029  & 0.08422538    \\
P100     & 9.526      & 2343835089  & 0.120317358   \\
P100     & 9.526      & 2915531621  & 0.14027827    \\
P100     & 9.526      & 10208089582 & 0.308935075   \\
K80      & 4.113      & 3943594121  & 0.445572447   \\
K80      & 4.113      & 4970946221  & 0.559733584   \\
K80      & 4.113      & 5882144461  & 0.654454093   \\
K80      & 4.113      & 663908170   & 0.231740283   \\
K80      & 4.113      & 5768251646  & 0.600807565   \\
K80      & 4.113      & 15906945758 & 1.217563636   \\
P100     & 9.526      & 3943594121  & 0.191349931   \\
P100     & 9.526      & 4970946221  & 0.23579211    \\
P100     & 9.526      & 5882144461  & 0.26991332    \\
P100     & 9.526      & 663908170   & 0.127421261   \\
P100     & 9.526      & 5768251646  & 0.235528539   \\
P100     & 9.526      & 15906945758 & 0.412028919   \\ \bottomrule
\end{tabular}
}
\end{table}

==> table_model_stats.tex <==
\begin{table*}[!]
    \centering
    \sf 
    \caption*{\textbf{Summary of CNN models used in the experiments.} Stats
    included are important features that we used later to construct predictive
    models.The first group of models is natively implemented in
    \texttt{Tensor2Tensor}, the second group customized for data collection. We
    altered two hyperparameters, hidden layer size and depth, to customize the
    second group of models. \tian{Can we replace all the N/A with the
    \emph{layer depth} (assuming that is what you referred to ) for ResNet? The column name can be "(Hidden) Layer Depth".}~\shijian{I wrote some text about couple of issues here, please see~\ncite{2019\_week40\_b}}}
    \label{tab:model_comp}
    \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{c|l rrrrrrr}
        \toprule
        \multicolumn{1}{l|}{}                                     & \textbf{Model}             & \multicolumn{1}{l}{\textbf{GFLOPs}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Checkpoint \\ (MB)\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Weight File \\ (MB)\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Index File\\ (KB)\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Meta File \\ (MB)\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Hidden Layer \\ Size\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Hidden Layer \\ Depth\end{tabular}}} \\ \hline
        {\color[HTML]{656565} }                                   & \textbf{ResNet-15}         & 0.59                                & 6.27                                                                                    & 5.3                                                                                      & 5.42                                                                                   & 0.97                                                                                   & (2,  2,  2)                                                                               & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{ResNet-32}         & 1.54                                & 15.99                                                                                   & 14.19                                                                                    & 11.05                                                                                  & 1.79                                                                                   & (5, 5, 5)                                                                                   & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{Shake Shake Small} & 2.41                                & 26.39                                                                                   & 22.36                                                                                    & 22.07                                                                                  & 4.01                                                                                   & 32                                                                                        & 26                                                                                         \\
        \multirow{-4}{*}{{\color[HTML]{656565} \textbf{Base}}}    &
        \textbf{Shake Shake Big}   & 21.29                               &
        204.04
        & 200.01
        & 22.44
        & 4.01
        & 96
        & 26
        \\ \hline  
        \rule{0pt}{3ex} 
        {\color[HTML]{656565} }                                   & \textbf{Shake Shake 1}     & 0.62                                & 9.57                                                                                    & 5.64                                                                                     & 21.03                                                                                  & 3.91                                                                                   & 16                                                                                        & 26                                                                                         \\
        {\color[HTML]{656565} }                                   & \textbf{ResNet 1}          & 0.8                                 & 9.26                                                                                    & 8.12                                                                                     & 6.71                                                                                   & 1.13                                                                                   & (2, 3, 3)                                                                                   & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{ResNet 2}          & 1.01                                & 10.57                                                                                   & 9.25                                                                                     & 7.9                                                                                    & 1.31                                                                                   & (2, 5, 3)                                                                                   & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{ResNet 3}          & 1.44                                & 12.78                                                                                   & 11.09                                                                                    & 10.41                                                                                  & 1.68                                                                                   & (3, 8, 3)                                                                                   & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{ResNet 9}          & 1.86                                & 19.21                                                                                   & 17.15                                                                                    & 12.91                                                                                  & 2.05                                                                                   & (6, 6, 6)                                                                                   & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{ResNet 4}          & 2.72                                & 22.45                                                                                   & 20.12                                                                                    & 14.82                                                                                  & 2.32                                                                                   & (7, 7, 7)                                                                                   & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{ResNet 5}          & 2.72                                & 28.7                                                                                    & 25.9                                                                                     & 17.94                                                                                  & 2.78                                                                                   & (8, 9, 9)                                                                                   & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{Shake Shake 5}     & 3.05                                & 26.39                                                                                   & 22.36                                                                                    & 22.07                                                                                  & 4.01                                                                                   & 32                                                                                        & 32                                                                                         \\
        {\color[HTML]{656565} }                                   & \textbf{ResNet 6}          & 3.67                                & 38.85                                                                                   & 35.22                                                                                    & 23.61                                                                                  & 3.61                                                                                   & (10, 13, 12)                                                                                & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{ResNet 10}         & 3.99                                & 40.41                                                                                   & 36.49                                                                                    & 25.49                                                                                  & 3.89                                                                                   & (11, 15, 12)                                                                                & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{ResNet 7}          & 4.63                                & 48.15                                                                                   & 43.68                                                                                    & 29.26                                                                                  & 4.44                                                                                   & (14, 15, 15)                                                                                & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{ResNet 8}          & 5.48                                & 54.26                                                                                   & 49.05                                                                                    & 34.36                                                                                  & 5.18                                                                                   & (16, 20, 16)                                                                                & N/A                                                                                        \\
        {\color[HTML]{656565} }                                   & \textbf{Shake Shake 2}     & 5.37                                & 54.19                                                                                   & 50.16                                                                                    & 22.13                                                                                  & 4.01                                                                                   & 48                                                                                        & 26                                                                                         \\
        {\color[HTML]{656565} }                                   & \textbf{Shake Shake 3}     & 9.51                                & 93.33                                                                                   & 89.03                                                                                    & 22.39                                                                                  & 4.01                                                                                   & 64                                                                                        & 26                                                                                         \\
        {\color[HTML]{656565} }                                   & \textbf{Shake Shake 6}     & 12.06                               & 117.61                                                                                  & 112.71                                                                                   & 27.29                                                                                  & 4.87                                                                                   & 64                                                                                        & 32                                                                                         \\
        \multirow{-16}{*}{{\color[HTML]{656565} \textbf{Custom}}} & \textbf{Shake Shake 4}     & 14.81                               & 143.01                                                                                  & 138.98                                                                                   & 22.42                                                                                  & 4.01                                                                                   & 80                                                                                        & 26                                                                                         \\ 
        \bottomrule
        \end{tabular}}
\end{table*}
